An Extension of the Athena++ Framework for General Equations of State

We present modifications to the Athena++ framework to enable use of general equations of state (EOS). Part of our motivation for doing so is to model transient astrophysics phenomena, as these types of events are often not well approximated by an ideal gas. This necessitated changes to the Riemann solvers implemented in Athena++. We discuss the adjustments made to the HLLC, and HLLD solvers and EOS calls required for arbitrary EOS. We demonstrate the reliability of our code in a number of tests which utilize a relatively simple, but non-trivial EOS based on hydrogen ionization, appropriate for the transition from atomic to ionized hydrogen. Additionally, we perform tests using an electron-positron Helmholtz EOS, appropriate for regimes where nuclear statistical equilibrium is a good approximation. These new complex EOS tests overall show that our modifications to Athena++ accurately solve the Riemann problem with linear convergence and linear-wave tests with quadratic convergence. We provide our test solutions as a means to check the accuracy of other hydrodynamic codes. Our tests and additions to Athena++ will enable further research into (magneto)hydrodynamic problems where realistic treatments of the EOS are required.

==> tests/test_01_wave-speeds.tex <==
-7.0412538e-01 & 1.0725946e-01 & 5.9219500e-01 & 7.4980628e-01 & $-$

==> tests/test_02_wave-speeds.tex <==
-5.1742727e-01 & 6.5617334e-01 & 1.0452190e+00 & 1.1550984e+00 & $-$

==> tests/test_03_wave-speeds.tex <==
-1.8903927e-01 & $-$ & -5.6034656e-02 & 1.1655176e-01 & $-$

==> tests/test_04_wave-speeds.tex <==
-2.2343227e-01 & $-$ & -6.3748668e-02 & 1.4111796e-01 & $-$

==> tests/test_05_wave-speeds.tex <==
-1.1617972e+00 & -2.6033771e-01 & 0.0000000e+00 & 2.6033771e-01 & 1.1617972e+00

==> tests/test_06_wave-speeds.tex <==
-8.6273248e-01 & -1.0278163e-01 & 1.8235310e-01 & 4.6030997e-01 & 1.2617972e+00

==> tests/test_10_wave-speeds.tex <==
-1.0173409e+00 & 9.8304277e-02 & 9.0151646e-01 & 1.2833895e+00 & $-$

==> tests/test_11_wave-speeds.tex <==
-4.4550675e-01 & $-$ & -3.6430963e-02 & 4.4161443e-01 & $-$
